Boosting Object Representation Learning via Motion and Object Continuity

Recent unsupervised multi-object detection models have shown impressive performance improvements, largely attributed to novel architectural inductive biases. Unfortunately, they may produce suboptimal object encodings for downstream tasks. To overcome this, we propose to exploit object motion and continuity, i.e., objects do not pop in and out of existence. This is accomplished through two mechanisms: (i) providing priors on the location of objects through integration of optical flow, and (ii) a contrastive object continuity loss across consecutive image frames. Rather than developing an explicit deep architecture, the resulting Motion and Object Continuity (MOC) scheme can be instantiated using any baseline object detection model. Our results show large improvements in the performances of a SOTA model in terms of object discovery, convergence speed and overall latent object representations, particularly for playing Atari games. Overall, we show clear benefits of integrating motion and object continuity for downstream tasks, moving beyond object representation learning based only on reconstruction.

==> CRV.tex <==
\newcommand{\WS}[1]{\textcolor{blue}{\textbf{[WS: #1]}}}
\newcommand{\QD}[1]{\textcolor{green}{\textbf{[QD: #1]}}}

\begin{document}

\section{Conference TODOS}
\begin{enumerate}
    \item 1. A PDF document with the copyright form signed by the corresponding author. 

    \item 2. A PDF document with the final CRV of the paper for the post-proceedings. This PDF file will be used during the compilation of the code by Springer as sanity check for the final compiled paper version. The PDF file should be named sub\_<ID>.pdf, where ID is your paper ID .

    \item 3. A .zip file containing all the source files of the paper, namely, the text of the paper and all the illustrative materials (figures), so that the PDF can be fully re-compiled from the source files. Please ensure that the (sub)folder names within your zip files are not unnecessarily long. Overly-long folder names cause problems on certain Windows systems.
    
\end{enumerate}

\begin{enumerate}
    \item 1. You must use the Latex style from LNCS Springer page available at 
https://resource-cms.springernature.com/springer-cms/rest/v1/content/19238648/data/v6 (LaTeX) and https://resource-cms.springernature.com/springer-cms/rest/v1/content/19238706/data/v1 (Microsoft Word). Please consult Springer's authors' guidelines, available at 
https://www.springer.com/gp/computer-science/lncs/conference-proceedings-guidelines.

    \item The affiliated institutions, including town/city and country, are to be listed directly below the names of the authors. Multiple affiliations should be marked with superscript Arabic numbers, and they should each start on a new line. We encourage authors to insert their ORCIDs in superscripts next to their names.

    \item The maximum length of papers for the Research and the Applied Data Science Tracks is 14 pages for the technical content excluding references. The space for references is not limited. In addition, there is one page for the discussion of ethical issues (ethical statement).
    The maximum length of papers for the Demo Track is 4 pages for the technical content, not including references. The space for references is not limited. 

    \item Once the data processing is finished, Springer will send a copy of the final PDF of each paper to its corresponding author. The corresponding author is asked to check through the final PDF. If Springer does not receive a reply within the time frame given, then it is presumed that the author has found no errors in the paper. 
\end{enumerate}

\begin{enumerate}
    \item Please use as few LaTeX files as possible and name the main file clearly, e.g., main.tex, so it is clear to other people how the source should be compiled. Ideally, ensure that it is possible to compile your paper using pdflatex main.tex.
    Authors should supply the bib file including the references, as this file will be used by Springer to create the bbl file. Make sure that there are no hyperlinks in the references. 

    \item Please use the \tocauthor and \toctitle fields, as these are important to create the publication's Table of Contents.

    \item Please make sure that your paper is properly formatted. DO NOT change the format required by Springer or their style sheets. Do not reduce spaces, fonts, or anything else, and avoid self-defined environments. Springer will remove all LaTeX instructions that change their format, and the paper length will be judged by whatever remains. Note that the contribution will be compiled from the sources, not from your PDF, and your contribution may look entirely different in the end, if you modify the formatting. For more thoughts on this matter, see https://wires.onlinelibrary.wiley.com/doi/full/10.1002/widm.1361.

    \item Good scientific research and continued scientific progress rely on the 
    availability of data and code for follow-up research. We therefore ask 
    you to:
    1) make your code and data publicly available to the extent possible;
    2) add links (e.g. URL in a footnote) to it in the paper at the relevant 
    places.
    In the case your paper has any supplementary material, you can upload them online (e.g., GitHub repository or personal webpage), and provide a link to it in the paper.
\end{enumerate}

\section{Reviews}



\end{document}
